THINK-Bench: Evaluating Thinking Efficiency and Chain-of-Thought Quality of Large Reasoning Models

Large reasoning models (LRMs) have achieved impressive performance in complex tasks, often outperforming conventional large language models (LLMs). However, the prevalent issue of overthinking severely limits their computational efficiency. Overthinking occurs when models generate excessive and redundant tokens that contribute little to accurate outcomes, especially in simple tasks, resulting in a significant waste of computational resources. To systematically investigate this issue, we introduce Think-Bench, a benchmark designed to evaluate the reasoning efficiency of LRMs. We also propose novel efficiency metrics and conduct a comprehensive evaluation of various LRMs across multiple dimensions, including the reasoning process, outcome quality, and chain-of-thought (CoT) characteristics. Our analysis reveals that most LRMs exhibit overthinking in handling easy questions, generating unnecessarily lengthy reasoning chains. While many LRMs demonstrate high CoT quality, several suffer from low efficiency. We hope that Think-Bench can serve as a robust foundation for advancing research into LRMs.

==> table/statistics.tex <==
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{lc}
    \toprule
    Statistic  & Number \\
    \midrule
    Total questions & 1375 \\
      -Choice questions & 929 \\
      -Free-form questions & 446 \\
      -Math questions & 293 \\
      -Physics questions & 590 \\
      -Chemistry questions & 492 \\
    \midrule
    Total key step annotation & 13311 \\
      -Average inference step & 9.68  \\
    \midrule
    Maximum question length & 1893 \\
    Maximum answer length & 372 \\
    Average question length & 422.42  \\
    Average answer length & 7.59  \\
    \bottomrule
    \end{tabular}%
  \label{tab:statistics}%
\end{table}%
